Chat-like Asserts Prediction with the Support of Large Language Model

Unit testing is an essential component of software testing, with the assert statements playing an important role in determining whether the tested function operates as expected. Although research has explored automated test case generation, generating meaningful assert statements remains an ongoing challenge. While several studies have investigated assert statement generation in Java, limited work addresses this task in popular dynamically-typed programming languages like Python. In this paper, we introduce Chat-like execution-based Asserts Prediction (\tool), a novel Large Language Model-based approach for generating meaningful assert statements for Python projects. \tool utilizes the persona, Chain-of-Thought, and one-shot learning techniques in the prompt design, and conducts rounds of communication with LLM and Python interpreter to generate meaningful assert statements. We also present a Python assert statement dataset mined from GitHub. Our evaluation demonstrates that \tool achieves 64.7\% accuracy for single assert statement generation and 62\% for overall assert statement generation, outperforming the existing approaches. We also analyze the mismatched assert statements, which may still share the same functionality and discuss the potential help \tool could offer to the automated Python unit test generation. The findings indicate that \tool has the potential to benefit the SE community through more practical usage scenarios.

==> implication.tex <==
\section{Discussion and Implications}
\label{sec:discussion}


==> methodBackup.tex <==
 \section{Methodology}
\label{sec:methodology} 

\begin{figure*}
% 	height=70mm
    \centering
	\includegraphics[width=0.95\textwidth]{figures/overviewNewV2.png}
	\caption{The overview of our approach \tool. }
	\label{fig:overview}
\end{figure*} 


In this section, we introduce \tool, a system that engages the LLM as a role of unit test expert, and designs prompts to initiate multiple rounds of conversation with the LLM to automatically generate the assert statements based on a given Python unit test. Fig.~\ref{fig:overview} illustrates the system overview of \tool. 
A test case from our Python dataset comprises the focal method, test method, and corresponding assert statements.
The multi-round communication with the LLM involves three phases. First, we create a greeting prompt to define the task and provide one sample test case, enabling the LLM to better understand the task. In the second phase, we incorporate the target test case into the query and wait for the initial round of predictions. In the third phase, we execute the predicted assert statements using a Python interpreter and, if any error messages arise, input these messages back into the LLM to request corrections to its predictions. By interacting with the LLM, \tool collects the automatically generated assert statements and complete the unit test case.
\chen{Annotate the section.}

\subsection{Data Extraction}
\label{sec:methodologyDataExtraction} 
% \chen{Not very important, maybe put it to the later part?}
Our goal is to generate assert statements in Python projects. As of March 2023, Python has been acknowledged as the most popular programming language by the TIOBE Programming Community Index~\cite{web:languageRanking}; however, previous works have not focused on the assert generation area in Python. Therefore, \tool begins by constructing a Python unit test dataset specifically for generating assert statements. In Fig.~\ref{fig:tapSample}, we provide an example of how a data entry in the dataset is structured and presented. A data entry consists of three main parts, the focal method, unit test, and assert statements. 

Given a project, \tool first identifies the unit test files from it. 
Unlike Java projects, where test methods normally start with $@Test$ annotation (inherent to the JUnit framework)~\cite{watson2020learning}, Python projects do not have a universal annotation for indicating test methods. Instead, they often rely on naming conventions and specific testing frameworks such as unittest. In Python, test methods are generally prefixed with $test$~\cite{trautsch2017there} and contained within files following the pattern $test\_module\_name.py$ or $module\_name\_test.py$. We follow this rule to extract unit test files.

Then, \tool tries to match the focal methods with the test methods. Inspired by focal method extraction for Java projects~\cite{watson2020learning, qusef2010recovering}, we identify the last method call from the same library or project before the assert statements as the focal method. In some cases, the method calls are embedded inside the assert statements as parameters, for example, the $process\_spider\_input$ in Fig.~\ref{fig:tapSample}. This approach might be considered controversial, as the parameter to be predicted is already present in the prompts. However, in real-world scenarios, developers typically have a clear understanding of the focal method. Consequently, we believe that incorporating the focal method information in the prompts closely aligns with developers' actual workflow and context, providing a more realistic and practical representation of the problem at hand. 

Finally, we extract the assert statements from the unit test and use $\langle AssertPlaceholder\rangle$ to replace the assert statements within the unit test code. To differentiate different assert statements in the same test case, we give incremental numbers to each of the statements. 
The detailed implementation is discussed in Section~\ref{sec:datasetCollection}. 
Overall, we collected 3,696 test methods within the dataset.



\begin{figure}[!ht]
\inputminted[mathescape,
              frame=lines,
              fontsize=\footnotesize,
              escapeinside=||]{python}{codeSamples/tapSample.m}
\caption{Example code after the data extraction.}
\label{fig:tapSample}
\end{figure}



\begin{figure*}
% 	height=70mm
    \centering
	\includegraphics[width=1\textwidth]{figures/promptDesign.pdf}
	\caption{Prompt templates and sample responses. \chen{Please refer to this figure multiple times in the main text as the illustration!}}
	\label{fig:samplePrompt}
\end{figure*} 

\subsection{Dialog Prompt Design and Management}
Following the data extraction, we facilitate multiple rounds of conversation with the LLM to simulate the chat experience. As shown in Fig.~\ref{fig:overview}, we introduce three types of prompt templates, which are \textit{greeting prompt}, \textit{query prompt}, and \textit{feedback prompt}. These prompts interact with the LLM sequentially, with the content varying based on the target unit test case and the LLM's response in each round of the conversation. In Fig.~\ref{fig:samplePrompt}, we present the three prompt templates with real samples from the dataset.

\textbf{Greeting Prompt} is the first prompt we sent to the LLM, which includes a persona message, a task explanation, and a sample sourced from the same project. The sample code is divided into four parts. The focal method consists of the original code extracted from the project source code. The unit test part contains the unit test code with the placeholder $\langle AssertPlaceholder\rangle$. \chen{Please use this to be more professional.}
Subsequently, we present the Chain of Thoughts (CoT) section, which elaborates on the rationale behind each assert statement to provide a better understanding of the test case. Finally, the generated assertions part features the actual assert statements.


\textbf{Query Prompt} is the one that has the targeted test cases and follows a similar structure to the sample part in the greeting prompt, albeit incomplete. Additionally, we add a brief description in the Chain of Thoughts (CoT) section to remind the LLM model of the task and guide it in generating assert statements corresponding to the number of placeholders. 


\textbf{Feedback Prompt} is an optional component used when the generated assertions from the query prompt do not match the actual ones and produce assert errors during execution. In such cases, \tool appends the error message to the feedback prompt, enabling the LLM to revise and correct its previous prediction. When constructing the feedback prompt, it is beneficial to include specific information regarding the errors encountered during execution, as well as suggestions or expectations for the corrected output. This approach helps the LLM to better understand the issues and identify areas for improvement. Without explicitly addressing the mistakes, the model may continue to maintain its original idea, leading to suboptimal results, which also is confirmed by other works~\cite{}.
% consider talk about made a mistake,,,,

\chen{I feel that greeting/query/feedback prompt above overlap much with the list below. What is the difference?}

\subsubsection{Persona-based Prompting}
During interactions with LLMs, users typically concentrate on a specific task within a single session. The persona-based prompting approach assigns a persona or role related to the task given to the LLM~\cite{white2023prompt}. By adopting a persona or role, the LLM can align its responses with the expertise, knowledge, and context associated with the given persona. This approach provides a clear framework and perspective for the LLM's response generation, ensuring that the output is more relevant and accurate for the specific task. In the official OpenAI gpt-3.5-turbo documents, they also ask users to have a system message to help set the behaviour of the assistant~\cite{}.

In this study, we instruct the LLM to assume the role of a Python unit testing expert to assist in completing the unfinished test method by generating assert statements. The first sentence introduces the LLM to its assigned role. Then, inspired by a popular repository~\cite{web:awesomprompts}, which has garnered over 58k stars, we include a task description paragraph. The description details the input, CoT steps to tackle the task, and the expected output, effectively guiding the LLM in producing the desired results.


\subsubsection{Chain-of-thought Prompting}
Recent research in prompt design has demonstrated that for complex tasks requiring multi-step reasoning~\cite{wei2022chain, zhang2022automatic, kojima2022large}, incorporating a rationale or key phrase can significantly enhance the performance of LLMs. This approach, called Chain-of-thought (CoT) prompting, is effective in guiding LLMs toward desired outputs. 
In our work, we adopt the design of CoT prompting strategies, by adding the guiding phrase and then following with rationale steps for generating the assert statements. This approach aims to harness the benefits of both strategies to enhance the LLM's ability to produce accurate results. To develop the manual instruction steps, we examined how developers write assert statements~\cite{}. The first step is to identify the test method and the focal method. Next, developers need to determine the parameters being tested and the assert type, e.g., asserting the parameter value, type/instance, or structural information. The final step entails reasoning the assert value and generating the corresponding statement. 
% By following these steps, we aim to provide the LLM with a clear and effective framework for generating assert statements.


\subsubsection{One-shot Learning}
% It indicates that with similar questions being sampled for test questions, Retrieval-Q-CoT is negatively affected by misleading by similarity~\cite{zhang2022automatic}.
%Prior to the LLM, fine-tuning is an important approach for models to achieve good performance in specific tasks~\cite{howard2018universal}. 
The LLM, such as GPT-3, can achieve state-of-the-art performance on a wide variety of tasks using only few-shot prompts, in which examples of solved tasks (shots) are included in the prompt~\cite{reynolds2021prompt}. 
\chen{This is not a related work, just say directly. No need to mention that} Specifically, Nashid et al.~\cite{} demonstrated with information retrieval and few shots learning, LLM can generate assert statements in Java. However, it requires a significant amount of annotated data. Besides, for dynamically-typed languages like Python, the way code is written and tested varies. 
In such cases, providing a higher number of shots might not always lead to better results, and may even negatively impact the LLM's ability to generate appropriate assert statements. \chen{Any evidence?}
\chen{This paragraph can be removed.}

Our approach adopts one-shot learning prompt to generate assert statements for Python projects, enabling the LLM to learn from a single example and adapt its response generation accordingly. This method considers Python's unique language characteristics and assumes that the writing style remains consistent across the same project. 
Therefore, while retrieving this one sample, we only look for the one test method that is within the same test class of the target test method as the sample. 
If there is only one test method in a class, we look for the closest test method. \chen{Why closest? Just one!, and select that one?}
When more than two test methods are present in a class, we compute the cosine similarity of the method names and select the most similar one.  After locating the sample code, we parse it into a format suitable for constructing the Greeting Prompt, as illustrated in Fig.~\ref{fig:samplePrompt}, and generate the corresponding CoT process.
% By leveraging one-shot learning, our approach minimizes the dependency on extensive annotated data, making it more practical and scalable for a wider range of applications. Additionally, this method ensures that the generated assert statements are both accurate and relevant to Python projects.
 
\subsubsection{Multi-assert Generation}
Different from single assert generation, when generating multi-assert statements using LLM, it is essential to maintain the appropriate sequence of assertions to effectively validate the code and prevent false positives or negatives that could arise from an incorrect order.
In our approach, we assign a numerical identifier to each assert placeholder within the test case, such as $\langle AssertPlaceholder2\rangle$. \chen{I think in the future improvement of this work, you should not include ID} Additionally, We include instructions, such as ``\textit{Please provide EXACTLY one assert statement for each $\langle AssertPlaceholder\rangle$ in the unit test case.}'', in both the greeting prompt and query prompt. This ensures that the output number of the assert statements is accurate. During the CoT prompting process, we apply the CoT to each AssertPlaceholder and sequentially generate the corresponding assertions, ensuring the preservation of the inline logic inherent to the test case code.


\subsection{Feedback Interaction}
Despite the LLM's ability to generate accurate assert statements, particularly with the CoT prompting which enables it to understand the testing purpose (derived from the test method and focal method names) and locate the parameter to be tested, there are instances where the LLM can not generate the correct value for the target parameters. For example, in situations where the target parameter value relies on complex math calculations (e.g., Deep learning models)~\cite{} or is influenced by external factors not immediately evident from the test method or focal method (e.g., global parameters, other util functions), the LLM may fail to deduce the correct value. 

To address this limitation, we introduce a feedback interaction that allows the LLM to learn from any execution errors it makes in generating the parameter values. Inspired by Ni et al.~\cite{ni2023lever}, we execute the generated assert statement in a Python Interpreter. As illustrated in Fig.~\ref{fig:overview}, the feedback coordinator \chen{Do we still have this? Try to align with your updated figure. And try not to create so many terms to make the paper as easy as possible to understand.} takes in the first-round generated assert statements and replaces them with the assert placeholders in the unfinished test case. Then, it will generate a temp file \chen{Too engineering, just say executate...}, save the Python test file to its project, and execute the test case with the Pytest library~\cite{}.
If the assert passed, the LLM has identified the correct value for the tested parameter. However, if the assert statement fails, we parse the error message from the Pytest library, which follows a specific pattern of providing information about the expected and actual values. This information is often presented in a comparison format, such as ``\textit{Expected= x, Actual= y, Details= ...}''. We then incorporate the error message into the feedback prompt, ensuring that the LLM is aware of its previous mistake and can use this information to adjust its response generation accordingly for the specific assert placeholder. By iterating through this feedback interaction, the LLM can progressively generate precise values for target parameters. After all interactions finish, \tool collects the second-round predictions and saves them for evaluation.





 
